Learned Score-Based Turbo Message Passing for Compressive Image Recovery

Score-based generative models have been incorpo-rated into message passing algorithms for compressive image recovery, providing a prior for the denoising module in message passing. Score-based generative models assume the input signal to be a clean signal perturbed by independent and identically distributed (i.i.d.) Gaussian noise. Yet, this assumption often fails during message passing, leading to slow convergence and limited reconstruction quality. In this letter, we propose the learned score-based turbo message passing (LSTMP) algorithm to overcome this limitation. By employing a deep unfolding framework, LSTMP unrolls the iterative process into a neural network, enabling the denoiser to adapt to complicated noise distributions inherent in the iterative updates. Furthermore, by treating the denoiser as an iterative solver, we incorporate the likelihood information of compressed measurements into the neural network of the denoiser, resembling the message passing between linear and nonlinear modules in STMP. Experiments on the FFHQ dataset show that LSTMP achieves convergence in no more than three iterations while delivering high-ffdelity re-constructions, signiffcantly outperforming the existing baselines.

==> backup.tex <==
\section{Residual Network for Deep Unfolding}

Before unfolding the STMP algorithm into a $T$-layer network, the score network is trained to remove Gaussian noise of varying degrees. In the first-order score model parameterized by $\bm{\theta}$, the loss function can be given as 
\begin{equation}
    \min_{\bm{\theta}} \mathbb{E}_{p(\tilde{x})} \left[ \left\| \bm{s_{\theta}}(\tilde{\bm{x}}, \sigma^2) - \nabla_{\tilde{\bm{x}}} \log p(\tilde{\bm{x}}) \right\|_2^2 \right],
    \label{eq:first score}
\end{equation}
We model $\tilde{\bm{x}}$ as a Gaussian perturbation of $\bm{x}$. Then $\tilde{\bm{x}}$ can be given as $\tilde{\bm{x}}= \bm{x}+ \sigma\bm{n}$. Substituting $\nabla_{\tilde{\bm{x}}} \log p(\tilde{\bm{x}} \mid \bm{x}) = -\frac{\tilde{\bm{x}} - \bm{x}}{\sigma^2}=-\frac{\bm{n}}{\sigma}$ into \eqref{eq:first score} yields

\begin{equation}
    \min_{\theta} \ell_1(\theta; \sigma) \triangleq \mathbb{E}_{p(\bm{x})p(\tilde{\bm{x}} \mid \bm{x})} \left[ \left\| \bm{s}_{\theta}(\tilde{\bm{x}}, \sigma^2) + \frac{\bm{n}}{\sigma} \right\|_2^2 \right],
    \label{first score simple2}
\end{equation}
where $\bm{n}$ refers to Gaussian noise.

Although deep unfolding can partially address the issue that the score function can only fit Gaussian noise, using such a Gaussian denoising network as the initial training point leads to a large number of training iterations and slow convergence. In order to accelerate convergence, we use a neural network to directly learn the real noise instead of Gaussian noise. The real noise in each layer of LSTMP is the difference between the extrinsic information passed from module A to module B and the ground-truth data, which is 
\begin{equation}
    \bm{r}=\bm{x}-\bm{x}^{ext}_A.
\end{equation}
So \eqref{first score simple} can be rewritten as 
\begin{equation}
    \min_{\theta} \ell_1(\theta; \sigma) \triangleq \mathbb{E}_{p(\bm{x})p(\tilde{\bm{x}} \mid \bm{x})} \left[ \left\| \bm{{s}_{\theta}}(\tilde{\bm{x}}, \sigma^2) -\bm{r} \right\|_2^2 \right].
    \label{residual network}
\end{equation}
We call $\bm{s_{\theta}}(\cdot)$ in \eqref{residual network} the residual network. 

In order to effectively use the physical information ${\bm{y},\,\bm{A}}$, we integrate the information into the NN layers in $\bm{s_{\theta}}(\cdot)$. Instead of simply appending the measurement at the input layer, we follow the approach of IDM, injecting the observed $\bm{y}$ and the measurement matrix $\bm{A}$ into the deep features of the network. For a deep feature $\mathbf{F}_{in} \in \mathbb{R}^{(H/r) \times (W/r) \times C}$, the injector measurement first transforms it into image space data $\bm{f}$, which can be given as
\begin{equation}
    \bm{f} = \mathrm{Conv}_1\left((\mathbf{F}_{in})_{\uparrow r}\right) \in \mathbb{R}^{H \times W \times 3} .
\end{equation}
We then perform a channel-wise concatenation of  $\bm{f}$, $\bm{A}^\top \bm{A} \bm{f}$, and $\bm{A}^\top \bm{y}$ and transform the data back into the feature domain.
\begin{equation}
    \mathbf{F}_{out} = \mathbf{F}_{in} + \left(\mathrm{Conv}_2\left([\bm{f}, \bm{A}^\top \bm{A} \bm{f}, \bm{A}^\top \bm{y}]\right)\right)_{\downarrow r}.
\end{equation}
The injectors enable $\bm{s_{\theta}}(\cdot)$ to integrate measurement information and image features during the denoising process, thereby improving denoising quality.

